Hypothesis Testing for Class-Conditional Noise Using Local Maximum Likelihood

In supervised learning, automatically assessing the quality of the labels before any learning takes place remains an open research question. In certain particular cases, hypothesis testing procedures have been proposed to assess whether a given instance-label dataset is contaminated with class-conditional label noise, as opposed to uniform label noise. The existing theory builds on the asymptotic properties of the Maximum Likelihood Estimate for parametric logistic regression. However, the parametric assumptions on top of which these approaches are constructed are often too strong and unrealistic in practice. To alleviate this problem, in this paper we propose an alternative path by showing how similar procedures can be followed when the underlying model is a product of Local Maximum Likelihood Estimation that leads to more flexible nonparametric logistic regression models, which in turn are less susceptible to model misspecification. This different view allows for wider applicability of the tests by offering users access to a richer model class. Similarly to existing works, we assume we have access to anchor points which are provided by the users. We introduce the necessary ingredients for the adaptation of the hypothesis tests to the case of nonparametric logistic regression and empirically compare against the parametric approach presenting both synthetic and real-world case studies and discussing the advantages and limitations of the proposed approach.

==> sections/notes.tex <==
\section{Notes}


\subsection{From \cite{wasserman2006all}}

starts at Eq. (5.111)

$Y$ has an exponential family distribution, given $x$, if:
\begin{equation*}
f(y \mid x)=\exp \left\{\frac{y \theta(x)-b(\theta(x))}{a(\phi)}+c(y, \phi)\right\}
\end{equation*}
for some functions $a(\cdot), b(\cdot)$ and $c(\cdot, \cdot)$. Here, $\theta(\cdot)$ is called the canonical parameter and $\phi$ is called the dispersion parameter. It then follows that
$$
\begin{aligned}
r(x) & \equiv \mathbb{E}(Y \mid X=x)=b^{\prime}(\theta(x)), \\
\sigma^{2}(x) & \equiv \mathbb{V}(Y \mid X=x)=a(\phi) b^{\prime \prime}(\theta(x)) .
\end{aligned}
$$
The usual parametric form of this model is
$$
g(r(x))=x^{T} \beta
$$
for some known function $g$ called the link function. The model
$$
Y \mid X=x \sim f(y \mid x), \quad g(\mathbb{E}(Y \mid X=x))=x^{T} \beta
$$

Let's consider a nonparametric version of logistic regression. For simplicity, we focus on local linear estimation. The data are $\left(x_{1}, Y_{1}\right), \ldots,\left(x_{n}, Y_{n}\right)$ where $Y_{i} \in\{0,1\}$. We assume that
$$
Y_{i} \sim \operatorname{Bernoulli}\left(r\left(x_{i}\right)\right)
$$
for some smooth function $r(x)$ for which $0 \leq r(x) \leq 1$. Thus, $\mathbb{P}\left(Y_{i}=1 \mid X_{i}=\right.$ $\left.x_{i}\right)=r\left(x_{i}\right)$ and $\mathbb{P}\left(Y_{i}=0 \mid X_{i}=x_{i}\right)=1-r\left(x_{i}\right)$. The likelihood function is
$$
\prod_{i=1}^{n} r\left(x_{i}\right)^{Y_{i}}\left(1-r\left(x_{i}\right)\right)^{1-Y_{i}}
$$
so, with $\xi(x)=\log (r(x) /(1-r(x)))$, the log-likelihood is:
$$
\ell(r)=\sum_{i=1}^{n} \ell\left(Y_{i}, \xi\left(x_{i}\right)\right)
$$
where
$$
\begin{aligned}
\ell(y, \xi) &=\log \left[\left(\frac{e^{\xi}}{1+e^{\xi}}\right)^{y}\left(\frac{1}{1+e^{\xi}}\right)^{1-y}\right] \\
&=y \xi-\log \left(1+e^{\xi}\right)
\end{aligned}
$$

To estimate the regression function at $x$ we approximate the regression function $r(u)$ for $u$ near $x$ by the local logistic function
$$
r(u) \approx \frac{e^{a_{0}+a_{1}(u-x)}}{1+e^{a_{0}+a_{1}(u-x)}}
$$
(compare with $(5.15))$. Equivalently, we approximate $\log (r(u) /(1-r(u)))$ with $a_{0}+a_{1}(x-u) .$ Now define the local log-likelihood
$$
\begin{aligned}
\ell_{x}(a) &=\sum_{i=1}^{n} K\left(\frac{x-X_{i}}{h}\right) \ell\left(Y_{i}, a_{0}+a_{1}\left(X_{i}-x\right)\right) \\
&=\sum_{i=1}^{n} K\left(\frac{x-X_{i}}{h}\right)\left(Y_{i}\left(a_{0}+a_{1}\left(X_{i}-x\right)\right)-\log \left(1+e^{a_{0}+a_{1}\left(X_{i}-x\right)}\right)\right)
\end{aligned}
$$
Let $\widehat{a}(x)=\left(\widehat{a}_{0}(x), \widehat{a}_{1}(x)\right)$ maximize $\ell_{x}$ which can be found by any convenient optimization routine such as Newton-Raphson. The nonparametric estimate
of $r(x)$ is
$$
\widehat{r}_{n}(x)=\frac{e^{\widehat{a}_{0}(x)}}{1+e^{\widehat{a}_{0}(x)}}
$$

\subsubsection{Model Selection}

\subsubsection{Other Issues (Section 5.13)}
\paragraph{Plug-In Bandwidth}
instead of using cross-validation to choose bandwidth, write down the formula for the asymptotically optimal bandwidth and then insert estimates of the unknown quantities in the formula.

\paragraph{Testing for linearity}
\todo[inline]{***}

\paragraph{Optimality}
\todo[inline]{***}

\todo[inline]{I don't think the following are needed but might be interesting for other reasons}

\paragraph{Derivative Estimation}
\paragraph{Variable Bandwidths and adaptive estimation}
\paragraph{Correlated data}
\paragraph{Robustness and Quantile Regression}
\paragraph{Measurement Error}

\subsubsection{Confidence Bands (Section 5.7)}
In this section we will construct confidence bands for $r(x)$. Typically these bands are of the form
$$
\widehat{r}_{n}(x) \pm c \operatorname{se}(x)
$$
where $\operatorname{se}(x)$ is an estimate of the standard deviation of $\widehat{r}_{n}(x)$ and $c>0$ is some constant. Before we proceed, we discuss a pernicious problem that arises whenever we do smoothing, namely, the bias problem.

THE BIAS PROBLEM. Confidence bands like those in $(5.97)$, are not really confidence bands for $r(x)$, rather, they are confidence bands for $\bar{r}_{n}(x)=\mathbb{E}\left(\widehat{r}_{n}(x)\right)$ which you can think of as a smoothed version of $r(x)$. Getting a confidence set for the true function $r(x)$ is complicated for reasons we now explain. Denote the mean and standard deviation of $\widehat{r}_{n}(x)$ by $\bar{r}_{n}(x)$ and $s_{n}(x)$. Then,
$$
\begin{aligned}
\frac{\widehat{r}_{n}(x)-r(x)}{s_{n}(x)} &=\frac{\widehat{r}_{n}(x)-\bar{r}_{n}(x)}{s_{n}(x)}+\frac{\bar{r}_{n}(x)-r(x)}{s_{n}(x)} \\
&=Z_{n}(x)+\frac{\operatorname{bias}\left(\widehat{r}_{n}(x)\right)}{\sqrt{\operatorname{variance}\left(\widehat{r}_{n}(x)\right)}}
\end{aligned}
$$
where $Z_{n}(x)=\left(\widehat{r}_{n}(x)-\bar{r}_{n}(x)\right) / s_{n}(x)$. Typically, the first term $Z_{n}(x)$ converges to a standard Normal from which one derives confidence bands. The second term is the bias divided by the standard deviation. In parametric inference, the bias is usually smaller than the standard deviation of the estimator so this term goes to zero as the sample size increases. In nonparametric inference, we have seen that optimal smoothing corresponds to balancing the bias and the standard deviation. The second term does not vanish even with large sample sizes.

The presence of this second, nonvanishing term introduces a bias into the Normal limit. The result is that
the confidence interval will not be centered around the true function $r$ due to the smoothing bias $\bar{r}_{n}(x)-r(x)$.

There are several things we can do about this problem. The first is: live with
it. In other words, just accept the fact that the confidence band is for $\bar{r}_{n}$ not $r$.There is nothing wrong with this as long as we are careful when we report the results to make it clear that the inferences are for $\bar{r}_{n}$ not $r$. A second approach is to estimate the bias function $\bar{r}_{n}(x)-r(x)$. This is difficult to do. Indeed, the leading term of the bias is $r^{\prime \prime}(x)$ and estimating the second derivative of $r$ is much harder than estimating $r$. This requires introducing extra smoothness conditions which then bring into question the original estimator that did not use this extra smoothness. This has a certain unpleasant circularity to it. ${ }^{6}$ A third approach is to undersmooth. If we smooth less than the optimal amount then the bias will decrease asymptotically relative to the variance. Unfortunately, there does not seem to be a simple, practical rule for choosing just the right amount of undersmoothing. (See the end of this chapter for more discussion on this point.) We will take the first approach and content ourselves with finding a confidence band for $\bar{r}_{n}$.

\subsection{From \cite{loader2006local}}
Local regression is used to model a relation between a predictor variable (or variables) $x$ and response variable $Y$, which is related to the predictor variables. Suppose a dataset consists of $n$ pairs of observations, $\left(x_{1}, Y_{1}\right),\left(x_{2}, Y_{2}\right), \ldots,\left(x_{n}, Y_{n}\right)$. We assume a model of the form
$$
Y_{i}=\mu\left(x_{i}\right)+\epsilon_{i}
$$
where $\mu(x)$ is an unknown function and $\epsilon_{i}$ is an error term, representing random errors in the observations or variability from sources not included in the $x_{i}$.

The errors $\epsilon_{i}$ are assumed to be independent and identically distributed with mean $0 ; \mathrm{E}\left(\epsilon_{i}\right)=0$, and have finite variance; $\mathrm{E}\left(\epsilon_{i}^{2}\right)=\sigma^{2}<\infty$. Globally, no strong assumptions are made about $\mu$. Locally around a point $x$, we assume that $\mu$ can be well approximated by a member of a simple class of parametric functions. For example, Taylor's theorem says that any differentiable function can be approximated locally by a straight line, and a twice differentiable function can be approximated by a quadratic polynomial. For a fitting point $x$, define a bandwidth $h(x)$ and a smoothing window $(x-h(x), x+h(x))$. To estimate $\mu(x)$, only observations within this window are used. The observations weighted according to a formula
$$
w_{i}(x)=W\left(\frac{x_{i}-x}{h(x)}\right)
$$

Within the smoothing window, $\mu(u)$ is approximated by a polynomial. For example, a local quadratic approximation is
$$
\mu(u) \approx a_{0}+a_{1}(u-x)+\frac{1}{2} a_{2}(u-x)^{2}
$$
whenever $|u-x|<h(x)$. A compact vector notation for polynomials is
$$
a_{0}+a_{1}(u-x)+\frac{1}{2} a_{2}(u-x)^{2}=\langle a, A(u-x)\rangle
$$
where $a$ is a vector of the coefficients and $A(\cdot)$ is a vector of the fitting functions. For local quadratic fitting,
$$
a=\left(\begin{array}{l}
a_{0} \\
a_{1} \\
a_{2}
\end{array}\right) \quad A(v)=\left(\begin{array}{c}
1 \\
v \\
\frac{v^{2}}{2}
\end{array}\right)
$$
The coefficient vector $a$ can be estimated by minimizing the locally weighted sum of squares:
$$
\sum_{i=1}^{n} w_{i}(x)\left(Y_{i}-\left\langle a, A\left(x_{i}-x\right)\right\rangle\right)^{2}
$$


\section{From \cite{frolich2006non}}
Fan and Gijbels (1996), Fan et al. (1998) and Carroll et al. (1998) $^{16}$ discuss estimation of bias and variance of the local likelihood estimator. A consistent estimator of the local variance of $\hat{\theta}_{x}$ can be obtained as
$$
\left(\sum \Lambda_{i} \bar{\Lambda}_{i} X_{i} X_{i}^{\prime} K_{i}\right)^{-1}\left(\sum\left(Y_{i}-\Lambda_{i}\right)^{2} X_{i} X_{i}^{\prime} K_{i}^{2}\right)\left(\sum \Lambda_{i} \bar{\Lambda}_{i} X_{i} X_{i}^{\prime} K_{i}\right)^{-1}
$$
where $\Lambda(u)=\frac{1}{1+e^{-u}}$ is the logit function and $\Lambda_{i}=\Lambda\left(X_{i}^{\prime} \hat{\theta}_{x}\right)$ and $\bar{\Lambda}_{i}=1-\Lambda_{i}$ and $\Lambda_{x}=\Lambda\left(x^{\prime} \hat{\theta}_{x}\right)$
and $\bar{\Lambda}_{x}=1-\Lambda_{x} \cdot{ }^{17}$ For a small sample size, Carroll et al. (1998) and Galindo et al. (2001) propose a degrees of freedom correction.

The variance approximation for $\hat{E}[Y \mid X=x]$ can then be obtained by the delta method as
$$
\operatorname{Var}(\hat{E}[Y \mid X=x]) \approx \Lambda_{x}^{2} \bar{\Lambda}_{x}^{2} \cdot x^{\prime} \widehat{\operatorname{Var}}\left(\hat{\theta}_{x}\right) x
$$

\section{Bootstrap correction}
\subsubsection{Bias Correction: Bootstrap}
Continuing with the parameter of interest from the previous section, we now discuss about the bias of the parameter: $\hat{\beta}$. The bias of a parameter is the difference between the mean as estimated from the sampling distribution, and the true value:
\begin{equation*}
    bias(\hat{\beta}) = \mathbb{E}\hat{\beta} - \beta
\end{equation*}

If $bias(\hat{\beta}) = 0$ then the estimator is said to be unbiased. Another important quantity is the standard error of an estimate:
\begin{equation*}
    se(\hat{\beta}) = \sqrt{\mathbb{V}\hat{\beta}} = \sqrt{\mathbb{E}\hat{\beta}^2 - (\mathbb{E}\hat{\beta})^2}
\end{equation*}

\paragraph{Non-Parametric Bootstrap:}
\begin{enumerate}
    \item Obtain $\hat{\theta}_0$, from the original sample $\{(x_i, y_i)\}_{j=1}^{n}$,
    \item For $\{i=1;i\leq B;i\texttt{++}\}:$
    \begin{enumerate}
        \item Sample $n$ times \textbf{with replacement} from $\{(x_i, y_i)\}_{j=1}^{n}$ to create new sample $S_i$,
        \item Obtain $\hat{\beta}_i^*$ from the new sample $S_i$.
    \end{enumerate}
    
\end{enumerate}

\paragraph{Parametric Bootstrap:}
\begin{enumerate}
    \item Obtain $\hat{\theta}_0$, from the original sample $\{(x_i, y_i)\}_{j=1}^{n}$,
    \item For $\{i=1;i\leq B;i\texttt{++}\}:$
    \begin{enumerate}
        \item $\forall~j\in [n]$, sample new labels: $y_{i, j} \sim f(\hat{\theta}_0, x_j)$ to form $S_i$,
        \item Obtain $\hat{\beta}_i^*$ from the new sample $S_i$.
    \end{enumerate}
    
\end{enumerate}

We can then estimate the bias, $bias(\hat{\beta})$ with $bias_{BS}(\hat{\beta})$ as follows:
\begin{equation}
    bias_{BS}(\hat{\beta}) = \frac{1}{B}\sum_{i=1}^n \hat{\beta}_i^* - \hat{\beta}_0
\end{equation}

The assumption around this estimate

